Harnessing Large Language Models for Curated Code Reviews

In code review, generating structured and relevant comments is crucial for identifying code issues and facilitating accurate code changes that ensure an efficient code review process. Well-crafted comments not only streamline the code review itself but are also essential for subsequent tasks like code refinement, where the code is modified to satisfy the input review comment. Although various AI-based approaches aimed to automate comment generation, their effectiveness remains limited by the quality of the training data. Existing code review datasets are often noisy and unrefined, posing limitations to the learning potential of AI models and hindering the automation process. To address these challenges, we propose a curation pipeline designed to enhance the quality of the largest publicly available code review dataset. We begin by establishing an evaluation framework, incorporating specific criteria and categories to empirically study the initial quality of the dataset. Using a large language model (LLM)-driven approach, we then apply our curation pipeline to refine the dataset. A comparative analysis of the newly curated dataset, based on the same evaluation framework, demonstrates substantial improvements in the clarity and conciseness of the comments. Additionally, we assess the impact of the curated dataset on automating downstream tasks, specifically comment generation and code refinement. Our findings show that the curated dataset leads to enhanced model performance in generating more accurate comments. Curated comments are also more useful as they lead to more accurate code refinement.

==> sections/draft.tex <==
\begin{table}[!htbp]
  \centering
  \caption{Distribution of categories across the original dataset.}
  \label{tab:categories_distribution_}
  \begin{tabular}{>{\centering\arraybackslash}p{1.2cm} >{\centering\arraybackslash}p{2cm}*{2}{r}}
    \toprule
    \textbf{Category} & \textbf{Subcategory} & \textbf{Count} & \textbf{Percentage}\\
    \midrule
    \multirow{6}{*}{\textbf{Type}} & Refactoring & 141 408 & 80.07 \\
    & Bugfix & 32 852 & 18.60 \\
    & Testing & 4 276 & 2.42 \\
    & Logging & 1 150 & 0.65\\
    & Documentation & 7 438 & 4.21 \\
    & Other & 15 837 & 8.97 \\
    \midrule
    \multirow{4}{*}{\textbf{Nature}} & Descriptive & 29 625 & 16.77 \\
    & Prescriptive & 145 088 & 82.15 \\
    & Clarification & 57 098 & 32.33 \\
    & Other & 25 & 0.01 \\
    \midrule
    \multirow{2}{*}{\textbf{Civility}} & Civil & 174 447 & 98.77 \\
    & Uncivil & 2 166 & 1.23 \\
    \bottomrule
  \end{tabular}
\end{table}


\begin{figure*}[htbp]
    \centering
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/dists/relevance_init_dist.png}
        \caption{Distribution of the relevance scores}
        \label{fig:rel_dist_init}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/dists/clarity_init_dist.png}
        \caption{Distribution of clarity scores}
        \label{fig:cla_dist_init}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.3\textwidth}
        \centering
        \includegraphics[width=\textwidth]{figures/dists/conciseness_init_dist.png}
        \caption{Distribution of conciseness scores}
        \label{fig:con_dist_init}
    \end{subfigure}

    \caption{Cumulative distribution of the different scoring criteria across the initial dataset \mw{See Fig. 4}}
    \label{fig:scores_init_dist}
\end{figure*}









